Symplectic integrators for index one constraints

We show that symplectic Runge-Kutta methods provide effective symplectic integrators for Hamiltonian systems with index one constraints. These include the Hamiltonian description of variational problems subject to position and velocity constraints nondegenerate in the velocities, such as those arising in sub-Riemannian geometry and control theory.

==> circle_phase_space_variables_0_caption.tex <==
\caption{Some of the phase space variables for the bicycle trajectory
starting in a circle.  The solution for $p_\theta$ and $p_\phi$ suggest
a relative homoclinic orbit.}


==> circle_phase_space_variables_0_mod_caption.tex <==
\caption{Some of the phase space variables for the bicycle trajectory
starting in a circle when doing modulo arithmetic on the angle
variables.  This is slightly better, 11 circles instead of 15.}


==> circle_phase_space_variables_1_caption.tex <==
\caption{Some of the phase space variables for the bicycle trajectory
starting in a circle.  These angle variables are monotonically
increasing.}


==> lambdas_for_circle_caption.tex <==
\caption{The error in the $\lambda$'s for the circle trajectory.  Note
that there are many more steps than shown in
Fig.~\ref{fig:circle_trajectory}.  This shows that the
$\lambda$'s periodically return to their values for a circle.} 


==> matlab_error_caption.tex <==
\caption{Error compared to \textsc{matlab} \texttt{ode15s} solution.  Initial conditions
were $(x, y, \theta, \phi, p_x, p_y, p_{\theta}, p_{\phi}) = (0.3, 0, 0, \pi, 0,
1.09, 1)$, with $\boldsymbol{\lambda} = (0, -0,3)$, final time $10s$,
and travelling in no potential
field.  The solution agrees with the \textsc{matlab} solution.}


==> straight_line_caption.tex <==
\caption{Snapshots at every $600^\mathrm{th}$ step of the bicycle
starting at $(x, y, \theta, \phi, p_x, p_y, p_{\theta}, p_{\phi}) = (0.15, 0,
0, 1, 0, 0, 0)$, with $\Delta t = 0.01$, and travelling in no potential
field.  The bicycle stays straight.  The trajectory is  unstable and
eventually wanders from a straight path.}


==> sym_condition_caption.tex <==
\caption{The symplectic bilinear form error evaluated for 100 steps with $\Delta t = 0.1$.
The trajectories 
$\phi_{z_i}(n)$ for three
nearby initial conditions, $z_0$, $z_1$, and $z_2$, were calculated. The 
change in the symplectic form was estimated as
$u_n^T J v_n - u_0^T J v_0$ where $u_n =  \phi_{z_1}(n) -
\phi_{z_0}(n)$ and $v_n = \phi_{z_2}(n) - \phi_{z_0}(n)$. The initial points were
$z_0 = (0.15, 0, 0, \frac{\pi}{4}, 0, 1, 0, 0)$,
$z_1 = (0.1500000085, 1 \times 10^{-8}, -1 \times 10^{-8}, 0.785398145543, -1 \times 10^{-8}, 0.99999998, 1 \times 10^{-8}, -1 \times 10^{-8})$
and $z_2 = (0.1500000115, -1 \times 10^{-8}, 1 \times 10^{-8}, 0.785398181251, 1 \times 10^{-8}, 0.99999998, -1 \times 10^{-8}, -1 \times 10^{-8})$.  }



